OpTHyLiC: an Optimised Tool for Hybrid Limits Computation

A software tool, computing observed and expected upper limits on Poissonian process rates using a hybrid frequentist-Bayesian CLs method, is presented. This tool can be used for simple counting experiments where only signal, background and observed yields are provided or for multi-bin experiments where binned distributions of discriminating variables are provided. It allows the combination of several channels and takes into account statistical and systematic uncertainties, as well as correlations of systematic uncertainties between channels. It has been validated against other software tools and analytical calculations, for several realistic cases.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = OTH-CPC

default: pdflatex

latex:
	latex  ${BASENAME}
	latex  ${BASENAME}
	bibtex ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}

pdflatex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	bibtex    ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 


